Respiratory Disease Classification and Biometric Analysis Using Biosignals from Digital Stethoscopes

Respiratory diseases remain a leading cause of mortality worldwide, highlighting the need for faster and more accurate diagnostic tools. This work presents a novel approach leveraging digital stethoscope technology for automatic respiratory disease classification and biometric analysis. Our approach has the potential to significantly enhance traditional auscultation practices. By leveraging one of the largest publicly available medical database of respiratory sounds, we train machine learning models to classify various respiratory health conditions. Our method differs from conventional methods by using Empirical Mode Decomposition (EMD) and spectral analysis techniques to isolate clinically relevant biosignals embedded within acoustic data captured by digital stethoscopes. This approach focuses on information closely tied to cardiovascular and respiratory patterns within the acoustic data. Spectral analysis and filtering techniques isolate Intrinsic Mode Functions (IMFs) strongly correlated with these physiological phenomena. These biosignals undergo a comprehensive feature extraction process for predictive modeling. These features then serve as input to train several machine learning models for both classification and regression tasks. Our approach achieves high accuracy in both binary classification (89% balanced accuracy for healthy vs. diseased) and multi-class classification (72% balanced accuracy for specific diseases like pneumonia and COPD). For the first time, this work introduces regression models capable of estimating age and body mass index (BMI) based solely on acoustic data, as well as a model for sex classification. Our findings underscore the potential of intelligent digital stethoscopes to significantly enhance assistive and remote diagnostic capabilities, contributing to advancements in digital health, telehealth, and remote patient monitoring.

==> backup.tex <==

\vspace{-5mm}
\subsection{Preprocesssing}
Preprocessing plays a crucial role in readying data for feature extraction and analysis, forming the foundation for training classification models. The process entails cleaning, filtering, selecting, and adapting raw data to ensure efficient, balanced, and equitable extraction of features and patterns. In the proposed approach, we utilize audio signals captured with a contact-based stethoscope, which can vary in recording frequency based on the medical device specifications. Hence, downsampling the audio signals is performed to reduce the computational burden and storage requirements, allowing us to retain essential information while optimizing processing resources. To prepare for downsampling, we applied a Hamming windowed low-pass FIR filter to mitigate aliasing and reduce high-frequency noise. FIR filters were chosen due to their linear phase response, stability, and control over frequency domain characteristics, offering advantages over IIR filters in preserving timing relationships and minimizing phase distortion, important for the next step in the pipeline. Following filtering, our approach involves the application of Empirical Mode Decomposition (EMD), a data-adaptive multiresolution technique, to effectively decompose the audio signals into meaningful components. EMD has proven invaluable in the analysis of non-linear and non-stationary signals, such as those derived from physiological processes like heart rate, respiration, and danger signs of respiratory conditions. This technique offers the distinct advantage of disentangling signals into their constituent components at different resolutions, revealing underlying structures that might be obscured in the raw data. EMD operates by decomposing signals into Amplitude-Modulated Frequency-Modulated (AM-FM) components, known as Intrinsic Mode Functions (IMFs), as pioneered by Huang and colleagues (1998). Importantly, this process is signal-dependent, bypassing any assumptions about the signal's linearity and stationarity. EMD has showcased its efficacy across a range of non-linear and non-stationary signal analyses in diverse fields. 

Subsequent to individualized analysis of each Intrinsic Mode Function (IMF) signal derived through Empirical Mode Decomposition (EMD), the power spectral density of each IMF signal was meticulously computed. This rigorous spectral analysis enabled the identification and selection of IMFs that prominently exhibited energy within specific frequency bands associated with physiological phenomena. Notably, IMFs were chosen based on their energy concentration in frequency ranges proximate to the heart rate (1 to 5 Hz) and respiration (0.1 to 1.5 Hz), as well as those encompassing the 5 to 10 Hz and 10 to 20 Hz bands. Intriguingly, two distinct envelope signals were further generated from the selected IMFs to capture nuanced physiological dynamics. The first envelope signal, enriched with higher frequency components, effectively encapsulated respiration-related information, enabling the discernment of respiratory patterns within the audio signals. In contrast, the second envelope signal, hailing from an IMF boasting lower audible frequencies, encapsulated the distinctive rhythmic oscillations inherent to cardiac activity. This comprehensive approach culminated in the extraction of six distinctive signals, of which five inherently encapsulate physiological attributes, while the sixth retains its acoustical nature. These physiological signals are substantiated by their frequency energy concentrations, rendering them invaluable for accurate characterization and interpretation of the underlying physiological processes. Such refined signal extraction not only enriches the diagnostic potential of the audio recordings but also underscores the utility of a multimodal approach in deciphering complex physiological phenomena within auscultatory data. This is one of the main differences with similar approaches using EMD for sound-based signal decomposition \cite{Sibghatullah2021COPDdetection}.



% Preprocessing plays a crucial role in readying data for feature extraction and analysis, forming the foundation for training classification models. The process entails cleaning, filtering, selecting, and adapting raw data to ensure efficient, balanced, and equitable extraction of features and patterns. In the proposed approach, we utilize audio signals captured with a contact-based stethoscope, which can vary in recording frequency based on the medical device specifications. Hence, downsampling the audio signals is performed to reduce the computational burden and storage requirements, allowing us to retain essential information while optimizing processing resources. To prepare for downsampling, we applied a Hamming windowed low-pass FIR filter to mitigate aliasing and reduce high-frequency noise. FIR filters were chosen due to their linear phase response, stability, and control over frequency domain characteristics, offering advantages over IIR filters in preserving timing relationships and minimizing phase distortion, important for the next step in the pipeline. Following filtering, our approach involves the application of Empirical Mode Decomposition (EMD), a data-adaptive multiresolution technique, to effectively decompose the audio signals into meaningful components. EMD has proven invaluable in the analysis of non-linear and non-stationary signals, such as those derived from physiological processes like heart rate, respiration, and danger signs of respiratory conditions. This technique offers the distinct advantage of disentangling signals into their constituent components at different resolutions, revealing underlying structures that might be obscured in the raw data. EMD operates by decomposing signals into Amplitude-Modulated Frequency-Modulated (AM-FM) components, known as Intrinsic Mode Functions (IMFs), as pioneered by Huang and colleagues (1998). Importantly, this process is signal-dependent, bypassing any assumptions about the signal's linearity and stationarity. EMD has showcased its efficacy across a range of non-linear and non-stationary signal analyses in diverse fields. 

% Subsequent to individualized analysis of each Intrinsic Mode Function (IMF) signal derived through Empirical Mode Decomposition (EMD), the power spectral density of each IMF signal was meticulously computed. This rigorous spectral analysis enabled the identification and selection of IMFs that prominently exhibited energy within specific frequency bands associated with physiological phenomena. Notably, IMFs were chosen based on their energy concentration in frequency ranges proximate to the heart rate (1 to 5 Hz) and respiration (0.1 to 1.5 Hz), as well as those encompassing the 5 to 10 Hz and 10 to 20 Hz bands. Intriguingly, two distinct envelope signals were further generated from the selected IMFs to capture nuanced physiological dynamics. The first envelope signal, enriched with higher frequency components, effectively encapsulated respiration-related information, enabling the discernment of respiratory patterns within the audio signals. In contrast, the second envelope signal, hailing from an IMF boasting lower audible frequencies, encapsulated the distinctive rhythmic oscillations inherent to cardiac activity. This comprehensive approach culminated in the extraction of six distinctive signals, of which five inherently encapsulate physiological attributes, while the sixth retains its acoustical nature. These physiological signals are substantiated by their frequency energy concentrations, rendering them invaluable for accurate characterization and interpretation of the underlying physiological processes. Such refined signal extraction not only enriches the diagnostic potential of the audio recordings but also underscores the utility of a multimodal approach in deciphering complex physiological phenomena within auscultatory data. This is one of the main differences with similar approaches using EMD for sound-based signal decomposition \cite{Sibghatullah2021COPDdetection}.



\subsection{Feature extraction}
Following the preliminary preprocessing phase, the acquired biosignals undergo a systematic windowing procedure, which represents a pivotal step in the data processing pipeline. Employing this method, each biosignal is partitioned into discrete, contiguous windows, each spanning a precise interval of 10 seconds. To ensure thorough coverage and comprehensive analysis of the biosignal, these windows are incrementally shifted by a predefined temporal step, typically set at 1 second. This strategic choice of step size results in an overlapping arrangement between successive windows, achieving an overlap rate of approximately 90\%. This overlap rate is carefully selected to preserve critical information across the segmentation process, effectively mitigating the risk of information loss that might arise from overly narrow steps.

The subsequent phase in our methodological framework is devoted to the extraction of an expansive assortment of features from the segmented biosignals. While traditional analysis of biosignals often revolves around the extraction of statistical features, encompassing both temporal and frequency domains, our approach significantly extends this repertoire. Our feature extraction strategy encompasses a wide spectrum of parameters, embracing vital signs, physiological attributes, morphological traits, entropy-based features, as well as fractal and complexity attributes derived from comprehensive fractal analysis. Additionally, we incorporate Mel-Frequency Cepstral Coefficients (MFCC) features to encapsulate the acoustical characteristics of the signal.

This augmented feature set synergistically bolsters the capacity of our methodology in the identification of distinctive medical conditions or symptomatic patterns. By encapsulating a broader array of attributes intrinsic to the biosignals, our approach enhances the potential for uncovering intricate correlations and distinctive markers that hold diagnostic or prognostic significance. This comprehensive feature extraction process, combined with meticulous windowing, exemplifies our commitment to extracting the most salient and representative information from biosignals, with the ultimate goal of enabling accurate medical condition identification and insightful pattern recognition.

A comprehensive feature set of 550 attributes is extracted from the six distinct signals associated with each patient. These features span various categories, commencing with statistical parameters that encompass mean, minimum, maximum, standard deviation, dynamic range, signal-to-noise ratio, median, and quartiles. These are further augmented through the computation of additional time-domain and frequency-domain statistical attributes, including parameters like slope, total spectral power, energy, and autocorrelation across both the entire window and subwindows.

Fractal analysis features encompass Katz fractal dimension, Higuchi fractal dimension, Petrosian fractal dimension, and detrended fluctuation analysis (DFA) of the complete window, among others. Moreover, the mean of these fractal analysis features is calculated over sub-windows within the larger window. Entropy analysis features include permutation entropy, spectral entropy, approximate entropy, sample entropy, Hjorth activity, mobility, complexity, and zero-crossings count within the entire window. Complexity analysis integrates attributes such as complex tolerance, dimension, and delay.

In the domain of heart and respiration features, our methodology embraces the computation of up to 70 physiological attributes, predominantly focusing on Heart Rate Variability (HRV)-related indicators. These HRV-related attributes span time-domain, frequency-domain, and non-linear-domain categories, meticulously detailed in previous references. Time-domain HRV features center around inter-beat intervals (IBI), time intervals between successive heartbeats, and normal beat intervals (NN intervals).

For computations, we employed the Numpy Python library for statistical features, the Antropy Python package for fractal and entropy attributes, and the Neurokit2 and HeartPy Python libraries for HRV-related attributes. Additionally, we devised customized features related to breathing patterns and the differences between facial and thoracic biosignals, leveraging both time and frequency domains when both are accessible.

This multi-faceted feature extraction process yields a comprehensive and discriminative feature set, crucial for the precise identification and analysis of physiological conditions in our proposed methodology.


\subsection{Feature extraction}

Following the preliminary preprocessing phase, the acquired biosignals undergo a systematic windowing procedure, which represents a pivotal step in the data processing pipeline. Employing this method, each biosignal is partitioned into discrete, contiguous windows, each spanning a precise interval of 10 seconds. To ensure thorough coverage and comprehensive analysis of the biosignal, these windows are incrementally shifted by a predefined temporal step, typically set at 1 second. This strategic choice of step size results in an overlapping arrangement between successive windows, achieving an overlap rate of approximately 90\%. This overlap rate is carefully selected to preserve critical information across the segmentation process, effectively mitigating the risk of information loss that might arise from overly narrow steps.

The subsequent phase in our methodological framework is devoted to the extraction of an expansive assortment of features from the segmented biosignals. While traditional analysis of biosignals often revolves around the extraction of statistical features, encompassing both temporal and frequency domains, our approach significantly extends this repertoire. Our feature extraction strategy encompasses a wide spectrum of parameters, embracing vital signs, physiological attributes, morphological traits, entropy-based features, as well as fractal and complexity attributes derived from comprehensive fractal analysis. Additionally, we incorporate Mel-Frequency Cepstral Coefficients (MFCC) features to encapsulate the acoustical characteristics of the signal.

This augmented feature set synergistically bolsters the capacity of our methodology in the identification of distinctive medical conditions or symptomatic patterns. By encapsulating a broader array of attributes intrinsic to the biosignals, our approach enhances the potential for uncovering intricate correlations and distinctive markers that hold diagnostic or prognostic significance. This comprehensive feature extraction process, combined with meticulous windowing, exemplifies our commitment to extracting the most salient and representative information from biosignals, with the ultimate goal of enabling accurate medical condition identification and insightful pattern recognition.

A comprehensive feature set of 550 attributes is extracted from the six distinct signals associated with each patient. These features span various categories, commencing with statistical parameters that encompass mean, minimum, maximum, standard deviation, dynamic range, signal-to-noise ratio, median, and quartiles. These are further augmented through the computation of additional time-domain and frequency-domain statistical attributes, including parameters like slope, total spectral power, energy, and autocorrelation across both the entire window and subwindows.

Fractal analysis features encompass Katz fractal dimension, Higuchi fractal dimension, Petrosian fractal dimension, and detrended fluctuation analysis (DFA) of the complete window, among others. Moreover, the mean of these fractal analysis features is calculated over sub-windows within the larger window. Entropy analysis features include permutation entropy, spectral entropy, approximate entropy, sample entropy, Hjorth activity, mobility, complexity, and zero-crossings count within the entire window. Complexity analysis integrates attributes such as complex tolerance, dimension, and delay.

In the domain of heart and respiration features, our methodology embraces the computation of up to 70 physiological attributes, predominantly focusing on Heart Rate Variability (HRV)-related indicators. These HRV-related attributes span time-domain, frequency-domain, and non-linear-domain categories, meticulously detailed in previous references. Time-domain HRV features center around inter-beat intervals (IBI), time intervals between successive heartbeats, and normal beat intervals (NN intervals).

For computations, we employed the Numpy Python library for statistical features, the Antropy Python package for fractal and entropy attributes, and the Neurokit2 and HeartPy Python libraries for HRV-related attributes. Additionally, we devised customized features related to breathing patterns and the differences between facial and thoracic biosignals, leveraging both time and frequency domains when both are accessible.

This multi-faceted feature extraction process yields a comprehensive and discriminative feature set, crucial for the precise identification and analysis of physiological conditions in our proposed methodology.

% A robust feature set of 550 attributes is derived from the six patient-associated signals. Statistical features include mean, min, max, and others, expanded with time-domain and frequency-domain parameters. Fractal analysis covers dimensions like Katz, Higuchi, and Petrosian, with entropy metrics like permutation and spectral. Heart and respiration analysis spans 70 attributes, predominantly HRV-based, while custom features tackle breathing patterns and biosignal disparities. Libraries like Numpy, Antropy, Neurokit2, and HeartPy facilitate computations. This comprehensive feature extraction enhances our methodology's physiological condition identification and analysis.

==> notes.tex <==
%%%%%%%%%%%%%%%%%%
%
%  TINO NOTES - Based on Reviewers' comments
%
%%%%%%%%%%%%%%%%%


%########################
% R1Q2: 
%     I don't know if 80 subjects is a large number or not for a study like this.
%     And I don't know if the age range of the subjects is appropriate.
%     Do young and old experience fatigue differently?

%  POSSIBLE ANSWER:
%       In this study, we exclusively investigate a cohort of young and healthy subjects aged between 18 and 68 years, focusing on the correlation between thermal camera frames and exercise-induced fatigue levels. We recognize our investigation's limitations due to this specific demographic, acknowledging the potential for further exploration across various age and health conditions groups in future research. 

%   FIXED []
%########################



%########################
% R1Q3: 
%       So you are estimating "fatigue" from the pattern of blood flow on the face. And assuming that a certain heart rate induces fatigue in everyone, and that fatigue decays as the number of frames from that point in the same way in everyone. But a really fit person might hit the target heart rate easily and not be fatigued?
% And different people may have the exercise-induced blood flow pattern decay at different rates?

%   FIXED [X]
%   Already explained in some of the sections.
%########################



%########################
% R1Q4: 
%   what about facial hair on men? Does this skew the result? Can't you detect facial hair and glasses and just not use those regions?
%
%
%  POSSIBLE ANSWER:
%   FIXED []
%  
%########################
